Capacity Provisioning Motivated Online Non-Convex Optimization Problem with Memory and Switching Cost

An online non-convex optimization problem is considered where the goal is to minimize the flow time (total delay) of a set of jobs by modulating the number of active servers, but with a switching cost associated with changing the number of active servers over time. Each job can be processed by at most one fixed speed server at any time. Compared to the usual online convex optimization (OCO) problem with switching cost, the objective function considered is non-convex and more importantly, at each time, it depends on all past decisions and not just the present one. Both worst-case and stochastic inputs are considered; for both cases, competitive algorithms are derived.

==> Proofs.tex <==
\subsection{Proof of Theorem \ref{thm:main}}
To prove Theorem \ref{thm:main}, we will use the primal-dual scheme. 
Towards that end, we first rewrite problem \eqref{eq:probquad} by writing the total flow time as the sum of flow time of each job  as follows
%\begin{equation}
%\begin{array}{c l} \min &\bc^T \bx, \\
%\bA\bx &\ge \bb,\\
%x_i &\ge 0, \ \forall \ i,
%\end{array}
%\end{equation}

\begin{equation}\label{eq:probeq}
\begin{aligned}
& \underset{s(t)}{\min}
& & \sum_j \left(\sum_{t=a_j}^{d_j} s_j(t) \right) \frac{d_j-a_j}{w_j}+ \alpha \sum_{t}  (s(t)- s(t-1))^2 \\
& \text{}
& & \begin{aligned} \sum_{t=a_j}^{d_j} s_j(t)  & \ge w_j, \ \forall \ j, \\
 s_j(t) &\geq 0 \ \forall \ t, j, \\
  \sum_{j} s_j(t) &= s(t) \ \forall \ t, \\ 
   \sum_{\tau \le t} s(\tau) &\le \sum_{\tau\le t} w(\tau) \ \forall \ t,
 \end{aligned}
\end{aligned}
\end{equation}
%\begin{equation}\label{eq:probeq}
%\begin{array}{rrclcl}
%\displaystyle \min_{s(t)} & \multicolumn{3}{l}{ \sum_j \left(\sum_{t=a_j}^{d_j} s_j(t) \right) \frac{d_j-a_j}{w_j}+ \sum_{t}  (s(t)- s(t-1))^2}\\
%\textrm{s.t.} &\sum_{t=a_j}^{d_j} s_j(t) &\ge w_j,\\
%&s_j(t) &\geq 0,    \\
%& \sum_{j} s_j(t) &= s(t), \\
%& \sum_{\tau \le t} s(\tau) &\le \sum_{\tau\le t} w(\tau) \ \forall \ t,
%\end{array}
%\end{equation}
where $s_j(t) = 1$ if job $j$ is being processed at time $t$, and $0$ otherwise, and $s(t)$ is the total number of active servers at time $t$, and the constraint $\sum_{t=a_j}^{d_j} s_j(t) \ge w_j$ implies that job $j$ is eventually completed.

The Lagrangian dual function associated with \eqref{eq:probeq} is \newline
\begin{align*}\label{}
 \min_{s(t)} \cL(\lambda_j, \mu_j, \nu_t, \eta_t) & =  \min_{s(t)} \quad  \sum_j \left(\sum_{t=a_j}^{d_j} s_j(t)  \right) \frac{d_j-a_j}{w_j} + \alpha \sum_{t}  (s(t)- s(t-1))^2 \\ 
& \quad \quad + \sum_j \lambda_j \left(w_j - \sum_{t=a_j}^{d_j} s_j(t)\right)   + \sum_j \mu_j s_j(t) + \sum_t \nu_t (\sum_{j} s_j(t) - s(t)) \\
&\quad \quad+ \sum_t \eta_t \left(\sum_{\tau \le t} s(\tau) - \sum_{\tau\le t} w(\tau)\right).
\end{align*}
where  $\lambda_j, \mu_j,\nu_t$ and $\eta_t$ are the dual variables.
Note that $$   \sum_j \left(\sum_{t=a_j}^{d_j} s_j(t)  \right) \frac{d_j-a_j}{w_j}  + \alpha \sum_{t}  (s(t)- s(t-1))^2 + \sum_j \lambda_j \left(w_j - \sum_{t=a_j}^{d_j} s_j(t)\right)$$ is also equal to 
\begin{align}\nn 
\sum_j \lambda_j w_j-   \sum_{j}  \sum_{t=a_j}^{d_j} (s_j(t)- s_j(t-1))\left(\lambda_j - \alpha (s(t)-s(t-1))-  \frac{d_j-a_j}{w_j}\right) \\ \label{eq:dummy1}
- \sum_{j}  \sum_{t=a_j}^{d_j} s_j(t-1)\left(\lambda_j - \frac{d_j-a_j}{w_j}\right).
\end{align}

Recall that $\max_{\lambda_j, \mu_j, \nu_t, \eta_t} \min_{s(t)} \cL(\lambda_j, \mu_j, \nu, \eta_t)$ is a lower bound on the objective value of the primal problem \eqref{eq:probeq}. 
Thus, even if we consider a fixed value of  $\lambda_j, \mu_j, \nu_t, \eta_t$, $\min_{s(t)} \cL(\lambda_j, \mu_j, \nu_t, \eta_t)$ is a lower bound on the objective value of the primal problem. In particular, we will make the following choices, $\mu_j=\nu_t=0, \eta_t=0\ \forall \ j,t$. How to choose $\lambda_j$ will be defined next.

Using \eqref{eq:dummy1}, and setting dual variables $\mu_j=\nu_t=0, \eta_t=0 \ \forall \ j, t$,  we get 
$\min_{s(t)} \cL (\lambda_j, \mu_j=0, \nu_t=0, \eta_t=0)  $
\begin{align}\nn  & =  \sum_{j } \lambda_j w_j - \max_{s(t)}  \left[\sum_{j}  \sum_{t} (s_j(t)- s_j(t-1)) 
 \left(\lambda_j - \alpha (s(t)-s(t-1))-  \frac{d_j-a_j}{w_j}\right) \right. \\ \label{eq:lbdual1} 
 & \quad \quad + \left.\sum_{j}  \sum_{t} s_j(t-1)\left(\lambda_j - \frac{d_j-a_j}{w_j}\right)\right].
\end{align}

{\bf Choosing the dual variable $\lambda_j$} Given the $\textsf{alg}$, choose $\lambda_j$ such that
$\lambda_j w_j = \Delta_j F$, where $\Delta_j F$ is the increase in the total flow time of the $\textsf{alg}$ because of arrival of job $j$ with size $w_j$ at time $a_j$, disregarding jobs arriving after time $a_j$.

For this choice of dual variables $\mu_j=\nu=\eta_t=0, \ \forall \ j$ and $\lambda_j$ as defined above, next, we will lower bound $$\min_{s(t)} \cL(\lambda_j, \mu_j=0, \nu_t=0, \eta_t=0)$$ and then use weak duality to derive a bound on the competitive ratio of the $\textsf{alg}$.


\begin{lemma}\label{lem:DeltaF} $\Delta_j F \le  ({\hat d}_j-a_j),$
where ${\hat d}_j$ is the completion time of job $j$ (following $\textsf{alg}$) assuming no further jobs arrive after job $j$.
\end{lemma}
\begin{proof} Note that with $\textsf{alg}$ the arrival of a new job does not decrease the number of active servers. Moreover, since all job sizes are equal and $\textsf{alg}$ is following multi-server SRPT, job $j$ does not preempt (block) any of the remaining jobs at time $t$ ever, and the increase in the total flow time is just the flow time of job $j$, i.e. ${\hat d}_j-a_j$.
%does not decrease the number of active servers with the $\textsf{alg}$. Thus, the total time for which job $j$ can block any other job from getting processed is at most $d_j-a_j$. Therefore, summing the flow time of $j$, i.e., $d_j-a_j$ and the cumulative increase in the flow time of all jobs because of job $j$, $d_j-a_j$, we get the result.
\end{proof}

Using Lemma \ref{lem:DeltaF} together with the definition of $\lambda_j w_j = \Delta_j F$, we get the following result.
\begin{lemma}\label{lem:lambdaj}
$\lambda_j \le  \frac{{\hat d}_j-a_j}{w_j}$ assuming that no new job arrives after time $a_j$.
\end{lemma}

\begin{remark} In contrast to ${\hat d}_j$, recall that $d_j$ is the actual completion time of job $j$ following $\textsf{alg}$ when jobs arrive after time $a_j$ as well. 
Instead of $\lambda_j \le  \frac{{\hat d}_j-a_j}{w_j}$ in Lemma \ref{lem:lambdaj}, if we had shown 
$\lambda_j \le  \frac{d_j-a_j}{w_j}$,  then we could have directly used that for analysis via bounding \eqref{eq:lbdual1}.  
Since more jobs can arrive after time $a_j$, $d_j\ne {\hat d}_j$. It is possible that $d_j< {\hat d}_j$, for example when more jobs arrive in near future, the number of active servers can be increased and it is possible that job $j$ might finish faster. %However, even that is not sufficient to claim that 
%$\lambda_j \le  \frac{d_j-a_j}{w_j}$. T
\end{remark}
To proceed further, next, we record an important property of the $\textsf{alg}$, for which we need the following definition.

\begin{definition}\label{defn:monotone} [Monotonicity] Consider two job arrival instances $\cI$ and $\cI'$ that are identical except that there is a single job $j \in \cI'\backslash \cI$. Moreover, assume that no job arrives after job $j$ that arrives at time $a_j$ in either $\cI$ or $\cI'$. Then an algorithm is defined to be {\bf monotone} if $n^{\cI}(t) \le n^{\cI'}(t)$, where $n^{\cI}(t)$ is the number of remaining jobs at time $t$ with job arrival instance $\cI$.
\end{definition}


\begin{lemma}\label{lem:monotone} $\textsf{alg}$ is monotone.
\end{lemma}
\begin{proof} 
From Definition \ref{defn:monotone}, for the two job arrival instances $\cI$ and $\cI'$, with $\textsf{alg}$ $n^{\cI}(t) = n^{\cI'}(t)$  for $t < a_j$, where $a_j$ is the arrival time of job $j$ under consideration.

Note that with $\textsf{alg}$, the arrival of new job cannot decrease the number of active servers. If the number of active servers remains the same with both $\cI$ and $\cI'$ throughout, then the claim follows directly. 

Thus, 
assume that the arrival of job $j$ increases the number of active servers $s(t)$ with the $\textsf{alg}$.  
Let job $j$'s arrival make $s(a_j) = s(a_j-1) + 1$. Thus, an additional server is now active compared to if job $j$ would not have arrived. 
Either job $j$ begins service on the newly active server, which means that there is no job that has arrived before job $j$ and  that is waiting at time $a_j$ to being serviced since all jobs are of equal size and multi-server SRPT is being executed. Thus, the arrival of new job has no effect on the completion time of any other outstanding job with the $\textsf{alg}$. 
Thus, given that 
$n^{\cI}(t) = n^{\cI'}(t)$  for $t< a_j$ by definition, we also have  $n^{\cI}(t) \le n^{\cI'}(t)$ for all $t$.

Now consider that case some other job (say $j'$) that is waiting at time $a_j-1$ begins service on the newly active server at time $a_j$. Then, from the choice of $s(t)$ made by $\textsf{alg}$, as soon as any one of the jobs that is under process at time $a_j$ is complete, the number of active servers reduces to $s(a_j-1)$ (or even lower if more than one jobs completes). Hence it is possible that job $j'$ completes faster because of the arrival of job $j$, however, in terms of the number of jobs in the system, $j$ has taken the place of $j'$ and we again get that $n^{\cI}(t) \le n^{\cI'}(t)$ for all $t$.
\end{proof}



Next, we show an important result that bounds the dual variable $\lambda_j$ in terms of the number of remaining jobs $n(t)$ at time $t$.


\begin{lemma}\label{lem:lambdajtime} For $\textsf{alg}$, $\lambda_j - \left(\frac{t-a_j}{w_j}\right) \le \frac{3}{\beta} (\alpha n(t))^{1/2}$ for all $t$ and $\beta^2\le 3$.
\end{lemma}

To prove Lemma \ref{lem:lambdajtime}, we will need the following intermediate result that bounds the flow time of job $j$ having size $w_j$ with $\textsf{alg}$ when $n-1$ other jobs arrive together with the $j^{th}$ job   at time $0$.


\begin{lemma}\label{lem:ubflowtime} Let $n$ jobs be available at time $0$, and the $j^{th}$ job among them be of size $w_j$. When no further job arrives after time $0$, then for the $\textsf{alg}$, job $j$'s flow time $f_j \le 3 w_j \sqrt{\alpha n}/\beta$ as long as $\beta^2\le 3$.
\end{lemma}
It is worth noticing that Lemma \ref{lem:ubflowtime} does not require all jobs to have the same size.

\begin{proof} Since the $\textsf{alg}$ uses multi-server SRPT for scheduling jobs and the number of active servers only depend on the number of remaining jobs, the worst case for maximizing the flow time of a job with size $w_j$ is when all other $n-1$ jobs are also of size $w_j$. In Proposition \ref{prop:ubcomptime}, we show that for the $\textsf{alg}$, when $n$ jobs of equal size $w$ are available at time $0$ and no further jobs arrive, all jobs are complete by at most time $\frac{3}{\beta} w \sqrt{n}$. This implies that job $j$ is complete by time $\frac{3}{\beta} w_j \sqrt{n}$ and the result follows.
\end{proof}


\begin{proposition}\label{prop:ubcomptime} Let at time $0$, the number of jobs be $n$ each with size $w$. When no further jobs arrive in future, with the $\textsf{alg}$ the time by which all jobs are finished is at most $\frac{3w}{\beta}\sqrt{\alpha n}$ when $\beta \sqrt{n/\alpha} = \min\{\beta \sqrt{n/\alpha}, n\}$ and $w$ otherwise.
\end{proposition}

\begin{proof} First consider $\beta=1$. How to extend it for general $\beta$ is detailed at the end.  Also, without loss of generality let $w=1$, since all jobs are of same size, we will simply scale the result by $w$.
We will prove the Proposition by showing the following two claims: i) $\textsf{alg}$ successively uses $L, L-1, L-2, \dots, 1 $ number of active servers, where $L = \lfloor\sqrt{n/\alpha}\rfloor$, and each number of active servers can be used for multiple consecutive time slots, and 
ii) the number of consecutive time slots for which a particular integral number of servers is used is at most $3$.

Note that by the definition of $\textsf{alg}$, the active number of servers chosen at the beginning is $L = \lfloor\sqrt{n/\alpha}\rfloor$.

To prove claim i), let time $t$ be the first time when the number of active servers is $q$ (some integer) with  the algorithm, and let $n(t)$ be the number of jobs at time $t$. 
Thus, we get that $n(t)/\alpha < (q+1)^2$ since otherwise the number of active servers chosen would have been $q+1$. 
Next, let $t'\ge t$ be the earliest time such that number of active servers $q$ becomes infeasible, i.e. with $t'-t=k$, 
$k$ is the smallest integer for which $n(t) - k q < \alpha q^2$. Therefore we get that $n(t) - (k-1) q \ge \alpha q^2$ which implies that 
$n(t) - k q \ge \alpha q^2 - q$. Since $\alpha q^2-q \ge \alpha (q-1)^2$ for $q\ge 1$, we get that $n(t) - k q \ge \alpha (q-1)^2$. Thus, at time $t'$ the number of active servers chosen is $(q-1)$.  
 
 For proving claim ii) again consider time $t$ where  $q$ (some integer) is the active number of servers chosen by the algorithm for the first time. Let $t'\ge t$ be the earliest time after $t$ where the number of active servers chosen by the algorithm is at most $q-1$. We want to show that $t'-t\le 3\alpha$. To prove this, suppose $t'-t>3 \alpha$. Then from time $t$ till $t'$ the number of active servers is $q$. By definition of time $t$, as above, we  get that  
$n(t)/\alpha < (q+1)^2$. Choosing active number of servers $q$ for $3\alpha$ consecutive slots, we get the number of jobs at slot $t+3$ to be $n(t) - 3\alpha q $ which is less than $\alpha q^2$ for any positive integer $q$, given that $n(t)/\alpha < (q+1)^2$. Thus at slot $t+3\alpha$ active number of servers  $q-1$ will be chosen, implying that $t'-t\le 3\alpha$.

Claim i) and ii) together imply that the total number of time slots needed to finish $n$ jobs of size $w$ (which is also the total flow time we are interested in) with $\beta=1$ is at most $3\sqrt{\alpha n} w$.  
%Thus, with general $\beta$, total number of time slots needed to finish $n$ jobs of size $w$ is at most is at most $\frac{3}{\beta} \sqrt{n} w$.

To extend the result for any $\beta>1$, note that when $\beta \sqrt{n/\alpha} = \min\{\beta \sqrt{n/\alpha}, n\}$,  the flow time upper bound (derived above) just  gets scaled by $\frac{1}{\beta}$. Let $n =  \min\{\beta \sqrt{n/\alpha}, n\}$. In this case, all $n$ jobs are processed simultaneously and the time by which all jobs will finish with $\textsf{alg}$ is $w$.\end{proof}



\begin{proof} [Proof of Lemma \ref{lem:lambdajtime}:]
From the monotone property of the $\textsf{alg}$ (Lemma \ref{lem:monotone}), it is sufficient to prove this result assuming that no job arrives after time $a_j$, the arrival time of job $j$ with size $w_j$. Also, recall that $\lambda_j w_j = \Delta_j F \le  {\hat d}_j-a_j$. Since no job arrives after job $j$, we also have  $d_j={\hat d}_j$. Moreover, from the fact that the $\textsf{alg}$ follows multi-server SRPT policy and the number of active servers only depend on the number of remaining jobs, the flow time of job $j$, $d_j-a_j$, is maximized if all the remaining jobs at time $a_j$ are of size $w_j$. Thus, we will consider this from here on. 

Let $S$ be the set of jobs remaining at time $a_j$ including $j$. Since job $j$ will finish the last as all the remaining jobs at time $a_j$ are of size $w_j$ and job $j$ has arrived the last,  with abuse of notation we let $|S|=j$. Consider time $t\ge a_j$, where $u-1$ jobs have been completed among $S$. Among the jobs in set $S$, let $d_i$ be the time of departure of the $i^{th}$ job in order. Then by the definition of $u$, we get that $[a_j, d_1) \cup [d_1, d_2) \cup \dots \cup [d_{u-2}, d_{u-1}) \subset [a_j, t]$. 

Thus \begin{equation}\label{eq:dummy2}
t-a_j \ge (d_1-a_j) + (d_2-d_1) +\dots + (d_{u-1}-d_{u-2}).
\end{equation}

From Lemma \ref{lem:lambdaj}, we have
$$\lambda_j - \frac{t-a_j}{w_j} \le \frac{ d_j-a_j}{w_j} - \frac{t-a_j}{w_j},$$
since $d_j={\hat d}_j$.

Using  \eqref{eq:dummy2}, we get that 

$$\lambda_j - \frac{t-a_j}{w_j} \le \frac{(d_j-d_{j-1}) + (d_{j-1}-d_{j-2}) +\dots + (d_{u}-d_{u-1})}{w_j}.$$
By definition of $u$, the number of jobs remaining at time $t$ is $n(t) = j-u+1$, and $(d_j-d_{j-1}) + (d_{j-1}-d_{j-2}) +\dots + (d_{u}-d_{u-1})$ is at most the time needed to finish 
$n(t) = j-u+1$ jobs of size at most $w_j$ each, with the $\textsf{alg}$. This time can be largest if the number of servers used by the $\textsf{alg}$ is $0$ at time $t$. Thus, applying Lemma \ref{lem:ubflowtime} where the initial number of active servers  is $0$, we get that $(d_j-d_{j-1}) + (d_{j-1}-d_{j-2}) +\dots + (d_{u}-d_{u-1}) \le \frac{3}{\beta} w_j \sqrt{\alpha (j-u+1)} = \frac{3}{\beta} w_j \sqrt{\alpha n(t)}$ as required.
\end{proof}
\newline

Now we are ready to lower bound the dual \eqref{eq:lbdual1}. By definition $ \lambda_j w_j = \Delta_j F$. Using this in  \eqref{eq:lbdual1}, we get 

$\min_{s(t)} \cL (\lambda_j, \mu_j=0, \nu_t=0, \eta_t=0) $
\begin{align}\nn 
& =  \sum_{j } \Delta_j F     - \max_{s(t)}  \left[\sum_{j}  \sum_{t} (s_j(t)- s_j(t-1)) 
 \left(\lambda_j -\alpha (s(t)-s(t-1))-  \frac{d_j-a_j}{w_j}\right) \right. \\ \nn & \quad \quad + \left.\sum_{j}  \sum_{t} s_j(t-1)\left(\lambda_j - \frac{d_j-a_j}{w_j}\right)\right], \\ \nn
 & =  \sum_{j } \Delta_j F     - \max_{s(t)}  \left[\sum_{j}  \sum_{t} (s_j(t)- s_j(t-1)) 
 \left(\lambda_j -\alpha (s(t)-s(t-1))-  \frac{d_j-a_j}{w_j}\right) \right].  
 \end{align}
 where the second equality follows since  for a fixed $j$,  $\sum_{t} s_j(t-1)=w_j$, and hence for a fixed $j$, 
 $$\sum_{t} s_j(t-1)\left(\lambda_j - \frac{d_j-a_j}{w_j}\right) = w_j \lambda_j - (d_j-a_j),$$ which upon using the fact that $ \lambda_j w_j = \Delta_j F$, implies that  $$ \sum_{j}  \sum_{t} s_j(t-1)\left(\lambda_j - \frac{d_j-a_j}{w_j}\right) = \sum_{j } \Delta_j F - \sum_j(d_j-a_j)  = F-F=0.$$
 Thus, again noting that $\sum_{j } \Delta_j F= F$, we get 
 $\min_{s(t)} \cL (\lambda_j, \mu_j=0, \nu_t=0, \eta_t=0) $
\begin{align}\nn 
& \stackrel{(a)}= F   - \max_{s(t)}  \left[  \sum_{j}  \sum_{t=a_j}^{d_j} (s_j(t)- s_j(t-1)) \left(\lambda_j - \alpha (s(t)-s(t-1))-  \frac{t-a_j}{w_j}\right)\right], \\ \nn 
& \stackrel{}= F   - \max_{s(t)}  \left[  \sum_{t=0}^{\infty} \sum_{j} (s_j(t)- s_j(t-1)) \left(\lambda_j -\alpha (s(t)-s(t-1))-  \frac{t-a_j}{w_j}\right)\right], \\ \nn 
%& = F    - \max_{s(t)}   \sum_{t=0}^{\infty} \sum_{j} (s_j(t)- s_j(t-1))\left(\lambda_j -(s(t)-s(t-1))-  \frac{t-a_j}{w_j}\right), \\ \nn
& \stackrel{(b)}\ge F   - \max_{s(t)} \left[  \sum_{t=0}^{\infty}  (s(t)- s(t-1))\left(\frac{3}{\beta} \sqrt{\alpha n(t)} - \alpha (s(t)-s(t-1))\right)\right], \\ \nn 
\end{align}
where $(a)$ follows from  the fact that for job $j$ the sum over time in the second term is for indices $t\le d_j$, and $(b)$ follows from Lemma \ref{lem:lambdajtime}.  Since $ (s(t)- s(t-1))\left(\frac{3}{\beta}\sqrt{\alpha n(t)} - \alpha (s(t)-s(t-1))\right)$ is maximized at  $(s(t)- s(t-1))= \frac{\sqrt{n(t)}}{\frac{2\beta\sqrt{\alpha}}{3}}$ we get that 
$$\max_{s(t)} (s(t)- s(t-1))\left(\frac{3}{\beta}\sqrt{\alpha n(t)} -\alpha(s(t)-s(t-1))\right) = 
 \frac{n(t)}{\left( \frac{2\beta}{3}\right)^2}.$$
 
 Thus, 
\begin{align}\nn 
\min_{s(t)} \cL (\lambda_j, \mu_j=0, \nu_t=0, \eta_t=0) & \ge F - \frac{9}{4\beta^2}\sum_t n(t),\\ \nn
& = F- \frac{9}{4\beta^2}F, \\ \label{eq:finalduallb}
& = F \left(\frac{4\beta^2-9}{4\beta^2}\right). 
\end{align}

Comparing \eqref{eq:finalduallb} with the upper bound on the cost of $\textsf{alg}$ derived in Lemma \ref{eq:costalg}, we complete the proof of Theorem \ref{thm:main} as follows.

From the weak duality, the primal value of \eqref{eq:probquad} is at least as much as the value of any dual feasible solution. Thus, the competitive ratio of 
any online algorithm $\cA$ is at most the ratio of an upper bound on the cost of $\cA$ and a lower bound on the dual feasible solution. Hence combining  \eqref{eq:finalduallb} and Lemma \ref{eq:costalg}, we get that the competitive ratio of $\textsf{alg}$ is at most 

$$\mu_{\textsf{alg}} \le \frac{1+2\beta^2}{\left(\frac{4\beta^2-9}{4\beta^2}\right)}.$$

For $\beta^2=3$, we get $$\mu_{\textsf{alg}} \le 7\times 4= 28,$$
while optimizing over $\beta$, we get that the optimal $\beta = 2.177$ and the competitive ratio is $19.95$.

\subsection{Proof of Theorem \ref{thm:special}}
Consider the case when all jobs arrive at the same time, i.e., $ a_j=a\ \forall \ j$, which without loss of generality be $a=0$.
As before, we let $\mu_j = 0, \forall \ j, \nu_t=0, \eta_t=0$.  But in contrast to the proof of Theorem \ref{thm:main} where the dual variable $\lambda_j$ was chosen as $\lambda_j w_j  = \Delta_j F$,
we now choose $\lambda_j$ differently. Given that all jobs are available at time $0$, following $\textsf{alg}$ that uses SRPT for scheduling, let $d_j$ be the departure time of $j$.
%and are of equal size, we 
%consider them in any arbitrary order. Following $\textsf{alg}$, with $n$ jobs of size $w$ available at time $0$, let $d_j$ be the departure time of $j$. 
Since no job arrives after time $0$, $d_j$ is in fact the true departure time.
For job $j$, define $\lambda_j = \frac{d_j-a_j}{w_j}$. 

% w = \lambda_j = \Delta_j F$.
%\begin{lemma}\label{lem:DeltaFspecial} $\Delta_j F \le  (d_j-a_j).$
%\end{lemma}
%\begin{proof}
%Since $\textsf{alg}$ follows multi-server SPRT, and all jobs are of same size, arrival of  job $j$ does not affect the flow time of any other job, and  the increase in the total flow time because of job $j$ is equal to the flow time of job $j$, $(d_j-a_j)$.
%\end{proof}

Recall that in in Lemma \ref{lem:lambdaj} we were able to show $\lambda_j \le \frac{({\hat d}_j-a_j)}{w_j}$  when jobs arrive over time. 
Using $\lambda_j = \frac{(d_j-a_j)}{w_j}$ in  \eqref{eq:lbdual1}, we get
$$\min_{s(t)} \cL (\lambda_j, \mu_j=0, \nu_t=0, \eta_t=0) $$
\begin{align}\nn
& =  \sum_{j } \lambda_j w_j   - \max_{s(t)}  \sum_{j}  \sum_{t=a_j}^{d_j} (s_j(t)- s_j(t-1))  \left(\lambda_j -\alpha(s(t)-s(t-1))-  \frac{(d_j-a_j)}{w_j}\right), \\ \nn
& \stackrel{(a)}=  \sum_j(d_j-a_j)  - \max_{s(t)}  \sum_{j}  \sum_{t=a_j}^{d_j} (s_j(t)- s_j(t-1))\left( - \alpha (s(t)-s(t-1))\right), \\  \nn
& = F - \alpha \max_{s(t)}   \sum_{t=0}^{\infty}  (s(t)- s(t-1))\left( -(s(t)-s(t-1))\right),\\ \label{eq:finalduallbspecial}
& \stackrel{(b)}\ge  F,
\end{align}
where $(a)$ follows since $\lambda_j =\frac{(d_j-a_j)}{w_j}$, and $(b)$ follows since $\max_{s(t)}   \sum_{t=0}^{\infty}  (s(t)- s(t-1))\left( -(s(t)-s(t-1))\right) \le 0$. 

From Lemma \ref{eq:costalg}, the cost of $\textsf{alg}$ is at most $(1+2\beta^2)F$. Combining this with \eqref{eq:finalduallbspecial}, the competitive ratio of $\textsf{alg}$ is at most $(1+2\beta^2)$. Choosing $\beta=1$,  the result follows.

In this section, we considered the worst-case input and proposed a simple algorithm and bounded its competitive ratio. An obvious question at this point is: can the competitive ratio performance be improved if the input is stochastic and not worst case. We tackle this challenge next, when the job arrival is Poisson and show that in fact the stochastic setting is much simpler to analyze and a $3$-competitive algorithm is easy to construct.




==> SimulationResults.tex <==
Linear Switching Cost

\alpha = 1;
arr_rate = [5 10 15 20]


Algorithm s(t) = n(t) 
cost/T = [7.50,  13.5661 19.43 25.21]


Algorithm Balance |s(t)-s(t-1)| = n(t)

cost/T = [7.57,  13.7, 19.56,  25.16]


Algorithm s(t) = n(t)/2

cost/T = [10.6,  20.98, 31.6, 41.84]


\alpha > 1 case
\alpha = 2

Balance Algorithm 1 s(t) = n(t) / alpha

cost/T = [11.751, 22.67 33.39 44.12 ]


Algorithm Balance 2  |s(t)-s(t-1)| = n(t)/alpha
cost/T = [9.89, 17.08 23.64 30.13]


Algorithm s(t) = n(t)/\alpha^{1/4}
cost/T = [9.3, 15.78 21.6 27.36 ]

\alpha > 1 case
\alpha = 4


Balance Algorithm 1 s(t) = n(t) / alpha

cost/T = [20.89, 41.64 63.22 82.7 ]


Algorithm Balance 2  |s(t)-s(t-1)| = n(t)/alpha
cost/T = [13.51, 22.6 30.72  38.35]

Algorithm s(t) = n(t)/\alpha^{1/4}
cost/T = [11.28, 18.05 24.63 31.39 ]


Quadratic Switching Cost
\alpha = 1
arr_rate = [5 10 15 20]

Paper's algorithm
beta = 1 [21.55 91.99 210.62 376.63]
beta = \sqrt{3}  [8.64 31.09 70.9 127.3831]
beta = 2 [8.87 24.63 53.83 96.53]
beta=4 [15.13  29.18  32.6 30.08] Reason that with higher arrival rate, pays switching cost less often but reduces flow time significantly.

\alpha = 2
arr_rate = [5 10 15 20]

Paper's algorithm
beta = 1 [41.04 178.33 411.16 732.84]
beta = \sqrt{3}  [14.77 63.06 142 252]
beta = 2 [11.5 46.7 106 192]
beta=4 [23.13 20.49  30.6 52 ] Reason that with higher arrival rate, pays switching cost less often but reduces flow time significantly.

Comparison between Paper's algorithm and Balance.
\alpha=1
arr_rate = [5 10 15 20]
Balance = [12.08 23.55 35.34 46.69]
Paper's algorithm beta = \sqrt{3}  [8.64 31.09 70.9 127.3831]
Paper's algorithm beta = 2 [8.87 24.63 53.83 96.53]

\alpha = 2
Balance = [16.75 32.3 48.47 63.07]
beta = \sqrt{3}  [14.77 63.06 142 252]
beta = 2 [11.5 46.7 106 192]
beta=4 [23.13 20.49  30.6 52 ] 

{\bf Extreme Case}
arr_rate = [1000]
beta = 2 [130590]
beta =sqrt{3} [153710]
beta = 4 [58463]
Balance  [35549] 






